RE-GAINS & EnChAnT: Intelligent Tool Manipulation Systems For Enhanced Query Responses

Large Language Models (LLMs) currently struggle with tool invocation and chaining, as they often hallucinate or miss essential steps in a sequence. We propose RE-GAINS and EnChAnT, two novel frameworks that empower LLMs to tackle complex user queries by making API calls to external tools based on tool descriptions and argument lists. Tools are chained based on the expected output, without receiving the actual results from each individual call. EnChAnT, an open-source solution, leverages an LLM format enforcer, OpenChat 3.5 (an LLM), and ToolBench's API Retriever. RE-GAINS utilizes OpenAI models and embeddings with a specialized prompt based on the $\underline{R}$easoning vi$\underline{a}$ $\underline{P}$lanning $(RAP)$ framework. Both frameworks are low cost (0.01\$ per query). Our key contribution is enabling LLMs for tool invocation and chaining using modifiable, externally described tools.

==> devrev_queries.tex <==
% don:core:dvrv-us-1:devo/0:issue/1
\begin{tabular}{ll}
\toprule
Query & Target \\
\midrule
Summarize issues similar to
\texttt{url} & \begin{verbatim}

[
{
"tool_name": "get_similar_work_items",
"arguments": [
{
"argument_name": "work_id",
"argument_value": "don:core:dvrv-us-1:devo/0:issue/1"
}
]
},
{
"tool_name": "summarize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[0]"
}
]
}
]
\end{verbatim} \\
What is the meaning of life? & \begin{verbatim}
[]
\end{verbatim} \\
Prioritize my P0 issues and add
them to the current sprint & \begin{verbatim}
[
{
"tool_name": "who_am_i",
"arguments": []
},
{
"tool_name": "works_list",
"arguments": [
{
"argument_name": "issue.priority",
"argument_value": ["p0"]
},
{
"argument_name": "owned_by",
"argument_value": ["$$PREV[0]"]
},
{
"argument_name": "type",
"argument_value": ["issue"]
}
]
},
{
"tool_name": "prioritize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[1]"
}
]
},
{
"tool_name": "get_sprint_id",
"arguments": []
},
{
"tool_name": "add_work_items_to_sprint",
"arguments": [
{
"argument_name": "work_ids",
"argument_value": "$$PREV[2]"
},
{
"argument_name": "sprint_id",
"argument_value": "$$PREV[3]"
}
]
}
]
\end{verbatim} \\
Summarize high severity tickets
from the customer
UltimateCustomer & \begin{verbatim}
[
{
"tool_name": "search_object_by_name",
"arguments": [
{
"argument_name": "query",
"argument_value": "UltimateCustomer"
}
]
},
{
"tool_name": "works_list",
"arguments": [
{
"argument_name": "ticket.rev_org",
"argument_value": ["$$PREV[0]"]
},
{
"argument_name": "ticket.severity",
"argument_value": ["high"]
},
{
"argument_name": "type",
"argument_value": ["ticket"]
}
]
},
{
"tool_name": "summarize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[1]"
}
]
}
]
\end{verbatim} \\
What are my all issues in the triage
stage under part FEAT-123?
Summarize them. & \begin{verbatim}
[
{
"tool_name": "who_am_i",
"arguments": []
},
{
"tool_name": "works_list",
"arguments": [
{
"argument_name": "stage.name",
"argument_value": ["triage"]
},
{
"argument_name": "applies_to_part",
"argument_value": ["FEAT-123"]
},
{
"argument_name": "owned_by",
"argument_value": ["$$PREV[0]"]
},
{
"argument_name": "type",
"argument_value": ["issue"]
}
]
},
{
"tool_name": "summarize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[1]"
}
]
}
]
\end{verbatim} \\
List all high severity tickets coming
in from slack from customer
Cust123 and generate a summary
of them. & \begin{verbatim}
[
{
"tool_name": "search_object_by_name",
"arguments": [
{
"argument_name": "query",
"argument_value": "Cust123"
}
]
},
{
"tool_name": "works_list",
"arguments": [
{
"argument_name": "ticket.rev_org",
"argument_value": ["$$PREV[0]"]
},
{
"argument_name": "ticket.severity",
"argument_value": ["high"]
},
{
"argument_name": "ticket.source_channel",
"argument_value": ["slack"]
},
{
"argument_name": "type",
"argument_value": ["slack"]
}
]
},
{
"tool_name": "summarize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[1]"
}
]
}
]
\end{verbatim} \\
Given a customer meeting
transcript T , create action items
and add them to my current sprint & \begin{verbatim}
[
{
"tool_name": "create_actionable_tasks_from_text",
"arguments": [
{
"argument_name": "text",
"argument_value": "T"
}
]
},
{
"tool_name": "get_sprint_id",
"arguments": []
},
{
"tool_name": "add_work_items_to_sprint",
"arguments": [
{
"argument_name": "work_ids",
"argument_value": "$$PREV[0]"
},
{
"argument_name": "sprint_id",
"argument_value": "$$PREV[1]"
}
]
}
]
\end{verbatim} \\
Get all work items similar to
TKT-123, summarize them, create
issues from that summary, and
prioritize them & \begin{verbatim}
[
{
"tool_name": "get_similar_work_items",
"arguments": [
{
"argument_name": "work_id",
"argument_value": "TKT-123"
}
]
},
{
"tool_name": "summarize_objects",
"arguments": [
{ 
"argument_name":  "objects", 
"argument_value":  "$$PREV[0]" 
}
]
},
{
"tool_name": "create_actionable_tasks_from_text",
"arguments": [
{
"argument_name": "text",
"argument_value": "$$PREV[1]"
}
]
},
{
"tool_name": "prioritize_objects",
"arguments": [
{
"argument_name": "objects",
"argument_value": "$$PREV[2]"
}
]
}
]
\end{verbatim} \\
\bottomrule
\end{tabular}

